Characterizing the SLOPE Trade-off: A Variational Perspective and the Donoho-Tanner Limit

Sorted l1 regularization has been incorporated into many methods for solving high-dimensional statistical estimation problems, including the SLOPE estimator in linear regression. In this paper, we study how this relatively new regularization technique improves variable selection by characterizing the optimal SLOPE trade-off between the false discovery proportion (FDP) and true positive proportion (TPP) or, equivalently, between measures of type I error and power. Assuming a regime of linear sparsity and working under Gaussian random designs, we obtain an upper bound on the optimal trade-off for SLOPE, showing its capability of breaking the Donoho-Tanner power limit. To put it into perspective, this limit is the highest possible power that the Lasso, which is perhaps the most popular l1-based method, can achieve even with arbitrarily strong effect sizes. Next, we derive a tight lower bound that delineates the fundamental limit of sorted l1 regularization in optimally trading the FDP off for the TPP. Finally, we show that on any problem instance, SLOPE with a certain regularization sequence outperforms the Lasso, in the sense of having a smaller FDP, larger TPP and smaller l2 estimation risk simultaneously. Our proofs are based on a novel technique that reduces a calculus of variations problem to a class of infinite-dimensional convex optimization problems and a very recent result from approximate message passing theory.

==> proof_mobius_sharp.tex <==
\section{Overcoming the Donoho-Tanner Power Limit}
\label{sec:app_sharp}

In what follows, we provide heuristic explanations for why SLOPE is able to overcome the upper bound on the TPP when the DT phase transition occurs, when the Lasso cannot. We first note that we will only consider the case where the $\tppinf$ is larger than $u_{\textnormal{DT}}^\star$ since achievability of  $\tppinf = u$ when $u < u_{\textnormal{DT}}^\star$ has already been shown using the Lasso in \cite[Lemma C.4]{lassopath}. Therefore this region is also achievable for SLOPE since Lasso is a special form of SLOPE.  

With this goal in mind, we begin by giving some intuition from an algorithmic perspective for why the Lasso has bounded TPP in some $(\delta,\epsilon)$ settings and then we will be prepared to discuss what makes SLOPE behave differently for \textit{arbitrary} priors.

First, recall that the Lasso sparsity ratio, i.e.\ the asymptotic proportion of non-zeros in the Lasso estimate, is upper bounded by $\delta = n/p$.  This illustrated in \cite[equation (C.1)]{lassopath}) where the result is proved using an  analysis via AMP, similar to ours. 

We now visualize this upper bound on the TPP step-by-step through the SLOPE proximal operation (which, of course, is the Lasso proximal operation when all threshold values are equal). This visualization will provide intuition for how SLOPE is different from the Lasso in terms of the sparsity of the estimator.  Before we do this, we review the SLOPE proximal operation.


Let $\bm s \in \R^\p$ be an input vector
% be defined as $\bm s=q_p(\Pi+\tau Z)$, the vector of $p$-quantiles of $\Pi+\tau Z$ \textcolor{dgreen}{for some $\tau > 0$,} at probabilities $\{\frac{1}{p+1},\cdots,\frac{p}{p+1}\}$, 
and let $\thet \in \R^\p$ %where $\bfalph$ and $\tau$ are determined by equations \eqref{eq:SE_finite} and \eqref{eq:cali_finite}.
be a vector of sorted penalties. The SLOPE proximal solution %, denoted as $\prox(\bm s;\thet)$, 
is defined as  
$$\prox(\bm s;\thet) = \argmin_{\bm b} \frac{1}{2}\|\bm{s}-\bm b\|^2+J_{\thet}(\bm b),$$
where  the definition of the slope penalty $J_{\thet}(\cdot)$ is given in \eqref{eq:SLOPE_penalty}.
One can find the solution $\prox(\bm s;\thet)$ in five steps as shown in \cite[Algorithm 3]{SLOPE1} and  restated here in Algorithm \ref{alg:prox}.



%\begin{algorithm}
%	\caption{Solving $\eta_{\text{soft}}(\bm s;\theta)$}
%	\begin{algorithmic}
%		\STATE (1). \textbf{Differencing:} Calculate  difference sequence, $\bm S$,
%		\begin{center}
%			$\bm S =\text{sort}(|\bm s|)-\thet$;
%		\end{center} 
%		\STATE (2). \textbf{Truncating:} Set negative values in the difference sequence to $0$: reassign 
%		\begin{center}
%			$\bm S =\max(\bm S,0)$;
%		\end{center}
%		\STATE (3). \textbf{Restoring:} Restore the sign of $\bm s$ from step (1) to $\bm S$.
%	\end{algorithmic}
%\end{algorithm}


% For example, to solve for $\prox([5,-7,3,0]; [6,2,2,1])$, step (1) sorts the first argument as $[7,5,3,0]$, recording the sign as $[-,+,+,+]$ and the order as $[2,1,3,4]$. Then step (2) gives the difference sequence as $[1,3,1,-1]$. Next, step (3) averages the first two entries and outputs $\AVE([1,3,1,-1])=[2,2,1,-1]$. Step (4) truncates the sequence to give $[2,2,1,0]$ and finally, step (5), restores the signs and orders to produce the outputs $[2,-2,1,0]$.

A typical plot of $\bm S$ after each step is shown in Figure~\ref{fig:Lasso not dense} for the Lasso. We note that step (3) of the algorithm has no effect and is therefore not represented in the plot. We remark that step (2) and (4) together have the soft thresholding effect of removing any non-zero entry from the solution if that entry falls between $[- \theta, \theta]$.  As a result, the solution is sparse.

%A typical plot of $\bm S$ after each step is shown in Figure~\ref{fig:Lasso not dense} for the Lasso, which is a sub-case of SLOPE where all elements of the penalty vector take the same value. In subplot (a), we plot the sorted $|\bm s|$ corresponding to step (1) in Algorithm ~\ref{alg:prox}. In subplot (b), we plot the output of step (2) of the algorithm: namely, we subtract $\thet$, a constant vector, so the result is just a downward shift of subplot (a).  In subplot (c), we perform step (4), the truncation, noting that for Lasso, step (3) of the algorithm has no effect and is therefore not represented in the plot. Finally, in subplot (d), we perform step (5) that restores the original signs and order.  Notice that step (2) and (4) together have the soft thresholding effect of removing any non-zero entry from the solution if that entry falls between $[- \lambda, \lambda]$.  As a result, the solution is sparse.

\begin{figure}[!htb]
	\centering
	\subfloat[after step (1)]{\includegraphics[width=0.25\linewidth]{LASSO1}}
	\subfloat[after step (2)]{\includegraphics[width=0.25\linewidth]{LASSO2}}
	\subfloat[after step (4)]{\includegraphics[width=0.25\linewidth]{LASSO3}}
	\subfloat[after step (5)]{\includegraphics[width=0.25\linewidth]{LASSO4}}
	\caption{A plot of the steps of the proximal operation as detailed in Algorithm~\ref{alg:prox},  in the case of Lasso  where the penalty vector $\thet$ takes a single value $2$. Here, $(\delta,\epsilon)=(0.3,0.2)$ and entries of $\bm s$ follow i.i.d. $\text{Bernoulli}(\epsilon)+\mathcal{N}(0,1)$.}
	\label{fig:Lasso not dense}
\end{figure}

%For comparison, in what follows we will plot the proximal steps for a two-level threshold SLOPE example, 
%like we for the Lasso in Figure \ref{fig:Lasso not dense}, 

%and discuss the reasons that SLOPE is able achieve full $\tppinf$ when Lasso cannot.  

%The plot uses $\alpha=2$ such that $\alpha\tau(\alpha)$ is roughly $3$, corresponding to $\lambda=2.2$. The setting is $(\delta,\epsilon)=(0.3,0.2)$ and $\Pi=2\cdot\text{Bernoulli}(\epsilon)$. 
%Notice that the quantiles of $\Pi+\tau Z$ have the smallest magnitude close to zero, as $\Pi+\tau Z$ is continuous and has range $(-\infty,\infty)$.




%\paragraph{SLOPE Can Achieve Any TPP.}
We now discuss why SLOPE can always achieve any TPP, given any prior, in any $(\delta,\epsilon)$ setting. We first discuss the special case of $\TPP=1$ since this special case is easy to understand and it motivates the strategy for demonstrating that SLOPE can achieve $\TPP \in (u_{\textnormal{DT}}^\star,1]$. 

First, by definition \eqref{TPP definition}, we must have $\TPP=1$ when $\widehat{\beta}_j\neq 0$ for all $j$, i.e. all predictors (including all the true ones) are selected.
%\begin{align*}
%\TPP(\blam)&=\frac{|\{j : \widehat{\beta}_j (\blam) \neq 0, \beta_j (\blam) \neq 0\}|}{|\{j : \beta_j(\blam) \neq 0\}|}.
%\end{align*}
Therefore, one way to achieve $\TPP=1$ is to find a SLOPE penalty $\blam$ for which the resulting estimator $\widehat\bet$ is completely dense. In fact, the connection between the sparsity of the estimator  $\widehat\bet$ and TPP proves vital in understanding the variable selection produced by SLOPE. %For now we consider constructing such a penalty and prior pair that gives $\TPP=1$.

Here, we consider a specific form of the two-level penalty vector, $\thet_{\lambda, 0,w}$, (recall $\thet_{\lambda_1, \lambda_2, w}$ was introduced in \eqref{eq:theta_func}) and we will argue that this penalty gives $\TPP=1$ for small enough $\lambda$ and $w$.
%\textcolor{dgreen}{when paired with a prior distribution of the form given in \eqref{eq:sharp_prior}}
%The idea is that this two-level penalty is constructed specifically to allow all entries in the solution to survive the thresholding (so that $\widehat\bet$ is completely dense, meaning $\TPP=1$).
This is done by not penalizing the weak magnitudes in the SLOPE solution at all and penalizing the stronger magnitudes only a little bit. One may view this special two-level SLOPE problem as a mixture of Lasso (with penalty $\lambda$) and ordinary least squares, the latter of which is always completely dense. In this setting, step (3) in Algorithm~\ref{alg:prox} plays an important role while step (4) has no effect, unlike the Lasso. This situation is demonstrated in Figure~\ref{fig:SLOPEtpp}. We notice that step (2) shifts the larger end of the curve down but leaves the smaller values unchanged, thus creating a vertical drop in the difference sequence which necessitates the averaging step (3). If the averaging terminates without alternating the smaller end of the curve, which is non-zero, the resulting estimator is then completely dense and hence $\TPP=1$.

%Again, in subplot (a), we plot the sorted $|\bm s|$ corresponding to step (1) in Algorithm~\ref{alg:prox}. In subplot (b), we plot the output of step (2) of the algorithm but now we subtract $\thet_p$, a two-level vector that shifts the larger end of the curve down but leaves the smaller values unchanged.  Notice that this creates a vertical gap due to the sudden drop in penalty strength from $\lambda$ to $0$.  In subplot (c), we perform the averaging step of the algorithm, step (3), and finally, in subplot (d), we perform step (5) that restores the original signs and order.  There is no step (4) here, because we purposely chose $\thet_p$ such that all elements are non-negative and none were thresholded.
%the output is completely dense: all elements are greater than or equal to 0 after step (3), so none were thresholded.
\begin{figure}[!htb]
	\centering
	\subfloat[after step (1)]{\includegraphics[width=0.25\linewidth]{SLOPE0}}
	\subfloat[after step (2)]{\includegraphics[width=0.25\linewidth]{SLOPE1}}
	\subfloat[after step (3)]{\includegraphics[width=0.25\linewidth]{SLOPE2}}
	\subfloat[after step (5)]{\includegraphics[width=0.25\linewidth]{SLOPE3}}
	\caption{A plot of the steps of the proximal operation as detailed in Algorithm~\ref{alg:prox},  in the case of SLOPE where the penalty vector $\thet=\thet_{1,0,0.2}$. Here, $(\delta,\epsilon)=(0.3,0.2)$ and entries of $\bm s$ follow i.i.d. $\text{Bernoulli}(\epsilon)+\mathcal{N}(0,1)$. None of the entries in $\prox(\bm s;\thet)$ is zero.}
	\label{fig:SLOPEtpp}
\end{figure}

%Considering Figure~\ref{fig:SLOPEtpp}, the reason that the two-level penalty $\thet_p(\lambda,0 ,w)$ successfully results in $\TPP=1$ when $w$ and $\lambda$ are  small enough, is that \textcolor{dgreen}{$\lambda$ is chosen smaller than $M$ given by \eqref{eq:sharp_prior} such that no values are shifted below $0$ in step (2)} and the averaging operation in step (3) that aims to level out the the vertical gap in the difference sequence $\bm S$, does not reach the rightmost element of the sequence $\text{sort}(|\bm s|)$. Importantly, after the averaging, the rightmost element of the sequence $\text{sort}(|\bm s|)$ can be close to zero, but will still be positive. %Given that the averaging stops if and only if the whole sequence is decreasing, we know that the sequence is positive. \cgr{I don't understand the previous sentence.} After restoring the order and signs, the sequence is completely dense and hence $\TPP=1$.


The key difference between SLOPE and Lasso proximal operations is through the averaging step, which is a direct consequence of using the sorted penalties. Indeed, when the averaging takes place, there will be groups of entries all sharing the same non-zero magnitude. On the other hand, both SLOPE and Lasso can select up to $n$ \textit{unique} magnitudes (see discussion about \eqref{finite_calibration}), but there is no mechanism to force any of the non-zero Lasso entries to take the same values. This causes the $\TPP$ limit to come into effect for the Lasso, while the entries of SLOPE estimator can be non-zero and not using up the uniqueness quota imposed by $\delta$.

%The key observation in the previous discussion for $\TPP=1$ is that the main difference between the SLOPE and Lasso proximal operations is through the averaging step, and it is through exploiting this averaging step that we can prove SLOPE achievability.  Indeed, when a SLOPE penalty has unequal levels, it causes the averaging to take place in step (3) and, as a result, there will be groups of entries all having the same non-zero magnitude. On the other hand, there is no mechanism to force any of the non-zero Lasso entries to take the same values and moreover, the number of non-zero Lasso entries is upper-bounded by $n$ as discussed previously.  This causes the $\TPP$ bound to come into effect for the Lasso. Through penalizing larger magnitudes more and smaller magnitudes less, some elements that would take zero values in the Lasso estimator will instead have non-zero magnitude in the SLOPE estimator.  This uses the fact that for SLOPE, only the number of \emph{unique} non-zero magnitudes is upper bounded by $n$, as opposed to the number  of non-zero elements, an idea we make rigorous in \eqref{C1b}.  

Motivated by the above ideas relating $\TPP$ and the estimator sparsity, in order to overcome the DT limit when considering $\TPP \in (u_{\textnormal{DT}}^\star,1)$, we design penalties such that a large number of $\widehat\beta_j$ share the same non-zero magnitude.  This is done by penalizing at two levels using $\bm\theta_{\lambda_1,\lambda_2,w}$, but with $\lambda_2>0$. As a result, we demonstrate in \Cref{sec:extend-donoho-tann} and \Cref{sec:slope-instance-better} that, with these two-level penalties, SLOPE can always overcome the Donoho-Tanner phase transition.

%Formally, we have the following result.

%Motivated by the above ideas relating $\TPP$ and estimator sparsity, in order overcome the DT limit when considering $\TPP \in (u_{\textnormal{DT}}^\star,1)$, we design penalties such that a large number of $\widehat\beta_j$ share the same non-zero magnitude.  This is done by penalizing at two levels and triggering the averaging step while still controlling the resulting sparsity, as in the $\TPP=1$ case.  Here we consider $\bm\theta(\lambda_1,\lambda_2,w)$, but with $\lambda_2>0$, because now we no longer want a completely dense estimator, but instead we want to use the fact that, unlike the Lasso, the proportion of non-zeros in the SLOPE estimator can exceed $\delta$.  In particular, this means that SLOPE can select more than $n = \delta p$ regressors and in order to drive the $\TPP^{\infty}$ up, we create penalty vectors that allow for a large number of the elements of $\widehat{\bet}$ to be non-zero. 

%\begin{fact}
%	Fix $\delta \in (0,\infty)$ and $\epsilon \in (0, 1)$ and let $\{\bet(\p)\}$ be an arbitrary prior sequence converging to a random variable $\Pi$. Then under the working hypotheses stated in \textbf{(A1)}-\textbf{(A3)}, any $0<u<1$ can be realized as $\tppinf$ by some $\{\blam(p)\}$ that converges to a bounded random variable $\Lambda$.
%	\label{lem:anyTPP}
%\end{fact}

%The proof is two-fold: for $0<u<u_{\textnormal{DT}}^\star$, the result is given in \cite[Lemma C.4]{lassopath}; for $u_{\textnormal{DT}}^\star<u<1$, the full proof is in Appendix \ref{app_sharp}. 





%To make this idea more clear, we introduce a new type of zero norm, $\|\cdot\|_0^*$, described also in the calibration formula of SLOPE AMP (see \cite{ourAMP}). In words, for a vector $\bm v$, the norm $\|\bm v\|_0^*$ counts the \emph{unique} non-zero magnitudes in $\bm v$ (as opposed to the standard zero norm $\|\bm v\|_0$ which instead counts every non-zero). For example, $\|(1,-1,0,2)\|_0^*=2$, while $\|(1,-1,0,2)\|_0=3$.  Then the SLOPE constraint is written as $\lim_p \frac{1}{p} \|\widehat\bet\|_0^*<\delta$, and notice that this returns the Lasso constraint too: since each entry in $\widehat\bet$ has a unique magnitude for Lasso, $\delta > \lim_p \frac{1}{p} \|\widehat\bet\|_0^*=\lim_p \frac{1}{p}\|\widehat\bet\|_0$.



%%% mode: latex
%%% TeX-master: "paper"
%%% End:

